Narratives: the Unforeseen Influencer of Privacy Concerns

Privacy requirements are increasingly growing in importance as new privacy regulations are enacted. To adequately manage privacy requirements, organizations not only need to comply with privacy regulations, but also consider user privacy concerns. In this exploratory study, we used Reddit as a source to understand users' privacy concerns regarding software applications. We collected 4.5 million posts from Reddit and classified 129075 privacy related posts, which is a non-negligible number of privacy discussions. Next, we clustered these posts and identified 9 main areas of privacy concerns. We use the concept of narratives from economics (i.e., posts that can go viral) to explain the phenomenon of what and when users change in their discussion of privacy. We further found that privacy discussions change over time and privacy regulatory events have a short term impact on such discussions. However, narratives have a notable impact on what and when users discussed about privacy. Considering narratives could guide software organizations in eliciting the relevant privacy concerns before developing them as privacy requirements.

==> extra.tex <==
% Recall in Section \ref{research_question_change} that we found privacy regulations related posts representing only a small minority of user privacy concerns expressed in Reddit. 
We grouped our data as a time series to see if privacy regulations impacted overall privacy concerns. 

For example, the GDPR came into full force in May 2018, but observing Figure \ref{fig:normalized_total_posts_no_general_over_time}, we see that there is little change in the number of privacy posts in the nearby months of May 2018. 
The number of privacy posts is hovering around the median level, significantly lower than the level observed in 2020 or 2021.
As discussed in Section \ref{research_question_change}, more GDPR related discussion occurred in the general privacy subreddits, and Figure \ref{fig:normalized_total_posts_only_general_over_time} reflects a slight increase of privacy posts between March to June 2018.
However, while the number of privacy posts during May 2018 was 50\% higher than the median, March to August 2018 were all at least 28\% higher than the median. 

We observed further that the total number of Reddit posts increased as time passed, which aligns with reports that more users joined Reddit the last few years \cite{kastrenakes_Reddit_2020}.
Also consistent with the total increase in Reddit post is the number of privacy posts. 
In fact, we can see from Figure \ref{fig:normalized_total_posts_no_general_over_time} where we normalized the count of privacy and non-privacy posts per month by their respective median that privacy has experienced significant growth over the past couple of years. 

It appears that the effect of the GDPR on the number of users discussing privacy posts is rather limited. 
Further to this point, the number of privacy posts regarding CCPA was even fewer than the GDPR so it too could not have drastically impacted user privacy discussion. 

Since January 2020 and culminating in January 2021, the monthly count of privacy related posts is repeatedly several times more than the median.
In January 2021, the number of privacy posts reached a new high of about five times the median value. 
While total posts on Reddit increased during this period, we can see from Figure \ref{fig:normalized_total_posts_no_general_over_time} that non-privacy posts did not increase the same magnitude.
The increase in the number of Reddit posts, particularly privacy related posts, was also found for the four general privacy subreddits as shown by Figure \ref{fig:normalized_total_posts_only_general_over_time}.
We observed that the change in the number of privacy posts was quite proportional to the non-privacy posts in Figure \ref{fig:normalized_total_posts_only_general_over_time}, but is more significant in 2020 and 2021. 

For both the general privacy subreddits and software product subreddits, we saw that the period with the largest increase in privacy posts was January 2021, but to our knowledge there were not any major privacy regulations that became law in that time interval that could have influenced an increase in privacy concern.
Since privacy regulatory changes could not explain spikes in privacy concern over time, we were motivated to further analyze what other potential contributing factors influenced user discussion regarding privacy. 



